ShiftAddAug: Augment Multiplication-Free Tiny Neural Network with Hybrid Computation

Operators devoid of multiplication, such as Shift and Add, have gained prominence for their compatibility with hardware. However, neural networks (NNs) employing these operators typically exhibit lower accuracy compared to conventional NNs with identical structures. ShiftAddAug uses costly multiplication to augment efficient but less powerful multiplication-free operators, improving performance without any inference overhead. It puts a ShiftAdd tiny NN into a large multiplicative model and encourages it to be trained as a sub-model to obtain additional supervision. In order to solve the weight discrepancy problem between hybrid operators, a new weight sharing method is proposed. Additionally, a novel two stage neural architecture search is used to obtain better augmentation effects for smaller but stronger multiplication-free tiny neural networks. The superiority of ShiftAddAug is validated through experiments in image classification and semantic segmentation, consistently delivering noteworthy enhancements. Remarkably, it secures up to a 4.95% increase in accuracy on the CIFAR100 compared to its directly trained counterparts, even surpassing the performance of multiplicative NNs.

==> tables/rebuttal_TVM.tex <==
\begin{table}[htbp]
  \setlength{\tabcolsep}{4pt}
  \centering
  % \vspace{-1.5em}
  \caption{Latency (ms) comparison with multiplication model on RTX 3090.}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{0.75\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \hline
    \hline
    \textbf{Method} & \textbf{MobileNetV2 w0.35} & \textbf{MobileNetV3 w0.35} & \textbf{MCUNet} & \textbf{ProxylessNAS w0.35} & \textbf{MobileNet-tiny} \\
    
    \hline
    \hline

    Baseline & 4.65 & 5.42 & 4.75 & 5.38 & 4.73 \\

    % \hline

    Shift & 1.35 & 2.24 & 1.55 & 1.62 & 1.36 \\

    % \hline

    Add & 3.76 & 4.93 & 4.68 & 5.19 & 3.864 \\
        
    \hline
    \hline
    \end{tabular}%
    }
  \label{tab:rebuttal_TVM}%
  \vspace{-0.5em}
\end{table}%

==> tables/rebuttal_convergence.tex <==
\begin{table}[ht]
    \vspace{-1.0em}
  \setlength{\tabcolsep}{4pt}
  \caption{The ablation study of different method for HWS}
  \centering
  % \caption{??????????????????????????}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \hline
    \hline
    \textbf{Method} & \textbf{MobileNetV2 w0.35} & \textbf{MobileNetV3 w0.35} & \textbf{MCUNet} & \textbf{ProxylessNAS w0.35} & \textbf{MobileNet-tiny} \\
    
    \hline
    \hline

    ShiftAddNAS & Nan & Nan & Nan & Nan & Nan \\

    Linear remap & Nan & Nan & Nan & Nan & Nan \\

    KL-loss only & 69.84 & 69.98 & 71.12 & 70.52 & 68.70 \\

    Linear + skip connect + freeze & 71.02 & 72.70 & 74.44 & 72.99 & 71.08 \\

    \hline
    
    \textbf{Ours} & 71.83 & 73.37 & 74.59 & 73.86 & 71.89 \\
    \hline
    \hline
    \end{tabular}%
    }
  \label{tab:rebuttal_convergence}%
  \vspace{0.0em}
\end{table}%

==> tables/rebuttal_inputReso.tex <==
\begin{table}[htbp]
  \setlength{\tabcolsep}{4pt}
  \centering
  % \caption{??????????????????????????}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \Xhline{3\arrayrulewidth}
    \textbf{Datasets} & \textbf{Method} & \textbf{Params(M)} & \textbf{Mult(M)} & \textbf{Shift(M)} & \textbf{Add(M)} & \textbf{Accuracy(\%)} & \textbf{MACs Saving(\%)}\\
    
    \hline
    \hline

    \multirow{2}*{CIFAR10} & ShiftAddNas-r32 & - & 17 & 19 & 58 & 95.83 & - \\
	                   ~ & ShiftAddAug-r96 & 2.05 & 12.3 & 14.5 & 28 & 95.92 & 40.4 \\

    \hline
    
    \multirow{4}*{CIFAR100} & ShiftAddNas-r32(multi-free) & - & 3 & 35 & 48 & 71.0 & - \\
                          ~ & ShiftAddNas-r32 & - & 22 & 21 & 62 & 78.64 & - \\
	                   ~ & ShiftAddAug-r160(multi-free) & 1.3 & 0.13 & 33.5 & 33.6 & 74.61 & 21.9 \\
                          ~ & ShiftAddAug-r96 & 2.3 & 16.2 & 20.2 & 36.4 & 78.72 & 33.8 \\
        
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
    }
  \label{tab:rebuttal_inputReso}%
  \vspace{-0.5em}
\end{table}%

==> tables/rebuttal_mIoU.tex <==
\begin{table}[htbp]
  \setlength{\tabcolsep}{4pt}
  \centering
  \caption{ShiftAddAug on OpenEDS dataset for semantic segmentation task}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{0.6\linewidth}{!}{
    \begin{tabular}{c|c|c}
    \hline
    \hline

    \textbf{Method} & \textbf{MobileNetV2 w0.35} & \textbf{ProxylessNAS w0.35} \\
    
    \hline
    \hline

    Base/NetAug & 88.68 / 92.41 & 86.27 / 92.84 \\

    Shift/\textbf{AugShift} & 88.01 / 94.52 & 86.01 / 95.12 \\

    Add/\textbf{AugAdd} & 83.94 / 91.20 & 82.01 / 90.45 \\
        
    \hline
    \hline

    \end{tabular}%
    }
  \label{tab:rebuttal_mIoU}%
  \vspace{-0.5em}
\end{table}%

==> tables/rebuttal_newTab.tex <==
\begin{table}[htbp]
  \setlength{\tabcolsep}{4pt}
  \centering
  % \caption{??????????????????????????}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
    \Xhline{3\arrayrulewidth}
    \textbf{Method} & \textbf{Backbone} & \textbf{Resolution} & \textbf{Params(M)} & \textbf{Mult(M)} & \textbf{Shift(M)} & \textbf{Add(M)} & \textbf{\makecell[c]{\textbf{CIFAR100}\\ \textbf{Accy(\%)}}} & \textbf{Energy(mj)} & \textbf{Latency(ms)} \\
    
    \hline
    \hline

    \multirow{8}*{\makecell[c]{DeepShift/\\ \textbf{AugShift}}} & MobileNetV2-w0.35 & 160 & 0.52 & 0 & 29.72 & 29.72 & 69.25 / \textbf{71.83} & 0.74 & 0.246 \\
                                                              ~ & MobileNetV2-w1.0 & 32 & 2.4 & 0 & 94.72 & 94.72 & 72.39 & 1.749 & 0.821 \\
                                                              ~ & MobileNetV2-Tiny & 160 & 0.35 & 0 & 27.31 & 27.31 & 68.29 / \textbf{71.89} & 0.697 & 0.228 \\
                                                              ~ & MobileNetV3-w0.35 & 160 & 0.96 & 0 & 18.35 & 18.35 & 68.42 / \textbf{73.37} & 0.536 & 0.16 \\
                                                              ~ & MCUNet & 160 & 0.59 & 0 & 65.72 & 65.72 & 70.87 / \textbf{74.59} & 1.323 & 0.545 \\
                                                              ~ & ProxylessNAS-w0.35 & 160 & 0.63 & 0 & 34.56 & 34.56 & 70.54 / \textbf{73.86} & 0.774 & 0.294 \\
                                                              ~ & ResNet-18 & 32 & 11.05 & 0 & 549.18 & 549.18 & 73.92 & 8.39 & 7.158 \\
                                                              ~ & VGG19 & 32 & 20.08 & 0 & 399.21 & 399.21 & 62.68 & 7.603 & 5.192 \\

    \hline

    \multirow{7}*{\makecell[c]{AdderNet/\\ \textbf{AugAdd}}} & MobileNetV2-w0.35 & 160 & 0.52 & 4.52 & 0 & 56.88 & 67.85 / \textbf{69.38} & 1.091 & 0.753 \\

                                                              ~ & MobileNetV2-Tiny & 160 & 0.35 & 4.43 & 0 & 52.09 & 66.57 / \textbf{67.65} & 0.999 & 0.693 \\
                                                              ~ & MCUNet & 160 & 0.59 & 20.91 & 0 & 113.09 & 70.25 / \textbf{72.72} & 2.345 & 1.72 \\
                                                              ~ & ProxylessNAS-w0.35 & 160 & 0.63 & 8.81 & 0 & 61.97 & 68.87 / \textbf{70.18} & 1.281 & 0.881 \\
                                                              ~ & ResNet-20 & 32 & 0.28 & 0.56 & 0 & 102.7 & 67.6 & 1.802 & 1.434 \\
                                                              ~ & ResNet-32 & 32 & 0.47 & 0.56 & 0 & 174.6 & 69.02 & 3.038 & 2.428 \\
                                                              ~ & VGG-small & 32 & 20.3 & 0 & 0 & 920 & 72.73 & 16 & 15.11 \\

    \hline

    \multirow{2}*{\makecell[c]{ShiftAddNet}} 

                                                                & ResNet-20 & 32 & 1.13 & 0 & 40.8 & 127.17 & 58.5 & 2.07 & 2.315  \\
                                                              ~ & VGG19 & 32 & 83.52 & 0 & 398 & 1380 & 65 & 24.68 & 25.632 \\

    \hline

    \multirow{2}*{\makecell[c]{ShiftAddNAS}} 

                                                                & mult-free & 32 & - & 3 & 35 & 48 & 71.0 & - & -  \\
                                                              ~ & hybrid & 32 & - & 22 & 21 & 62 & 78.6 & - & - \\

    \hline

    \multirow{2}*{\makecell[c]{\textbf{ShiftAddAug}}} 

                                                                & mult-free (NAS) & 160 & 1.3 & 0.13 & 33.5 & 33.6 & \textbf{74.61} & 0.851 & 0.264  \\
                                                              ~ & hybrid (NAS) & 96 & 2.3 & 16.2 & 20.2 & 36.4 & \textbf{78.72} & 2.431 & 0.644 \\

    
        
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
    }
  \label{tab:rebuttal_newTab}%
  \vspace{-0.5em}
\end{table}%

==> tables/rebuttal_tabFixRow.tex <==
\begin{table}[htbp]
  \setlength{\tabcolsep}{4pt}
  \centering
  % \caption{??????????????????????????}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
    \Xhline{3\arrayrulewidth}
    \textbf{Model} & \textbf{Method} & \textbf{Params(M)} & \textbf{Mult(M)} & \textbf{Shift(M)} & \textbf{Add(M)} & \textbf{Accuracy(\%)} & \textbf{Energy(mj)} & \textbf{Latency(ms)} \\
    
    \hline
    \hline

    ShiftAddAug & NAS & 1.90 & 0.13 & 33.50 & 33.60 & 74.61 & 0.851 & 0.264 \\
        
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
    }
  \label{tab:rebuttal_tabFixRow}%
  \vspace{-0.5em}
\end{table}%

==> tables/rebuttal_threeModel.tex <==
\begin{table}[htbp]
  \setlength{\tabcolsep}{4pt}
  \centering
  % \caption{??????????????????????????}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \Xhline{3\arrayrulewidth}
    \textbf{Method} & \textbf{MobileNetV2 w0.35} & \textbf{MobileNetV3 w0.35} & \textbf{MCUNet} & \textbf{ProxylessNAS w0.35} & \textbf{MobileNet-tiny} \\
    
    \hline
    \hline

    Shift & 51.92 & 54.19 & 56.45 & 55.40 & 48.92 \\

    % \hline

    Augshift & 53.86 & 56.07 & 57.34 & 56.30 & 50.00 \\
        
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
    }
  \label{tab:rebuttal_threeModel}%
  \vspace{-0.5em}
\end{table}%

==> tables/rebuttal_woWeightShare.tex <==
\begin{table}[htbp]
  \setlength{\tabcolsep}{4pt}
  \centering
  % \caption{??????????????????????????}
  \renewcommand{\arraystretch}{1.25} % increase vertical spacing
  \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \Xhline{3\arrayrulewidth}
    \textbf{Method} & \textbf{MobileNetV2 w0.35} & \textbf{MobileNetV3 w0.35} & \textbf{MCUNet} & \textbf{ProxylessNAS w0.35} & \textbf{MobileNet-tiny} \\
    \hline
    \hline

    direct trained & 69.25 & 68.42 & 70.87 & 70.54 & 68.29 \\
    \textbf{w/o. weight sharing} & \textbf{69.42} & \textbf{69.66} & \textbf{71.13} & \textbf{70.53} & \textbf{68.40} \\
    with weight sharing & 70.12 & 71.56 & 72.68 & 70.91 & 69.28 \\
        
    \Xhline{3\arrayrulewidth}
    \end{tabular}%
    }
  \label{tab:rebuttal_woWeightShare}%
  \vspace{-0.5em}
\end{table}%
